SciCat: A Curated Dataset of Scientific Software Repositories

The proliferation of open-source scientific software for science and research presents opportunities and challenges. In this paper, we introduce the SciCat dataset -- a comprehensive collection of Free-Libre Open Source Software (FLOSS) projects, designed to address the need for a curated repository of scientific and research software. This collection is crucial for understanding the creation of scientific software and aiding in its development. To ensure extensive coverage, our approach involves selecting projects from a pool of 131 million deforked repositories from the World of Code data source. Subsequently, we analyze README.md files using OpenAI's advanced language models. Our classification focuses on software designed for scientific purposes, research-related projects, and research support software. The SciCat dataset aims to become an invaluable tool for researching science-related software, shedding light on emerging trends, prevalent practices, and challenges in the field of scientific software development. Furthermore, it includes data that can be linked to the World of Code, GitHub, and other platforms, providing a solid foundation for conducting comparative studies between scientific and non-scientific software.

==> 6_FurtherimprovementsDataset.tex <==
\section{Future improvements}
% To address the issues highlighted in the limitations section, we aim 
% to focus future improvements on
%to raise awareness about the establishment of standardized guidelines for the README, encouraging developers to provide comprehensive and accurate information and encourage the citation of papers and grants.
We have tried our best to expand the initial sample size of the projects, by starting with a vast dataset of 131 million repositories, to help improve the representativeness of the dataset and alleviate the impact of selection bias. Using WoC data source mitigates concerns of selection bias from a particular platform to some level, as it integrates data from Github, GitLab, SourceForge, Bitbucket, and many other open-source platforms. To further mitigate this limitation, we will make efforts to diversify the dataset even more using other smaller curated platforms like institutional GitHub and GitLab orgs, and other institutional repos, enhancing the dataset to ensure that it better reflects the broader landscape of scientific software projects.  To address the limitations posed by the use of LLMs and their performance, in the future, we plan to use the keywords collected from our initial analysis to further refine and validate the dataset with a subsequent analysis or modeling. This approach aims to mitigate the inaccuracies arising from the current model's limitations. 
% We have taken steps to mitigate some of these limitations by starting with a vast dataset of 131 million repositories, which provides a broader representation of open-source projects and reduces the potential impact of selection bias. 
 It is also important to acknowledge that certain limitations, particularly those related to the quality of the README.md file and the accuracy of the LLM, may persist and require ongoing efforts to improve. Hence, we would consider supplementing the README.md analysis with additional contextual information, such as project documentation, source code, and user feedback for future improvements. In addition, we will aim to raise awareness about establishing standardized guidelines for the README.md, encouraging developers to provide comprehensive and accurate information and encourage the citation of papers and grants. Exploring alternative validation strategies, such as surveying project maintainers or users, to provide additional dataset validation, especially for projects with limited external references. 
 
 % Longitudinal studies tracking the evolution of scientific software projects should also be conducted to keep the dataset relevant and valuable over time. 
% Engaging with the scientific software development community for collaborative efforts can lead to ongoing enhancements, ensuring that the dataset remains a valuable resource for researchers and practitioners in the field. 
% Regular updates and maintenance should also be considered to reflect the dynamic nature of scientific software developments.



